A 1-mm spectral line survey toward GLIMPSE Extended Green Objects (EGOs)

A northern subsample of 89 Spitzer GLIMPSE extended green objects (EGOs), the candidate massive young stellar objects, are surveyed for molecular lines in two 1-GHz ranges: 251.5- 252.5 and 260.188-261.188 GHz. A comprehensive catalog of observed molecular line data and spectral plots are presented. Eight molecular species are undoubtedly detected: H13CO+, SiO, SO, CH3OH, CH3OCH3, CH3CH2CN, HCOOCH3, and HN13C. H13CO+ 3-2 line is detected in 70 EGOs among which 37 ones also show SiO 6-5 line, demonstrating their association to dense gas and supporting the outflow interpretation of the extended 4.5 um excess emission. Our major dense gas and outflow tracers (H13CO+, SiO, SO and CH3OH) are combined with our previous survey of 13CO, 12CO and C18O 1-0 toward the same sample of EGOs for a multi-line multi- cloud analysis of line width and luminosity correlations. Good log-linear correlations are found among all considered line luminosities, which requires a universal similarity of density and thermal structures and probably of shock properties among all EGO clouds to explain. It also requires that the shocks should be produced within the natal clouds of the EGOs. Diverse degrees of correlation are found among the line widths. However, both the line width and luminosity correlations tend to progressively worsen across larger cloud subcomponent size-scales, depicting the increase of randomness across cloud subcomponent sizes. Moreover, the line width correlations among the three isotopic CO 1-0 lines show data scatter as linear functions of the line width itself, indicating that the velocity randomness also increases with whole-cloud sizes and has some regularity behind.

==> tab4.tex <==
\begin{table*}
\centering
\begin{minipage}{160mm}
\caption{\label{tab4}Column density 
($10^{14}$cm$^{-2}$), excitation temperature (K), 
and the abundance ($10^{-9}$) of organic species 
CH$_3$OH, CH$_3$OCH$_3$, HCOOCH$_3$ and 
CH$_3$CH$_2$CN  in 37 strong emission EGOs that 
have their methanol lines at least tentatively 
detected. Also given are the source sizes 
($\arcsec$) estimated from {\it Spitzer IRAC} infrared source sizes. }
\footnotesize\rm
\begin{tabular*}{\textwidth}{lr|rrr|rrr|rrr|rr}
\hline
object        & Source        & \multicolumn{3}{c}{CH$_3$OH} & \multicolumn{3}{c}{CH$_3$OCH$_3$} & \multicolumn{3}{c}{HCOOCH$_3$} & \multicolumn{2}{c}{CH$_3$CH$_2$CN} \\
              & size          & \multicolumn{3}{c}{---------------------} & \multicolumn{3}{c}{---------------------} & \multicolumn{3}{c}{---------------------} & \multicolumn{2}{c}{---------------------} \\
              &  
              & 
$T_{\rm ex}$  & $N_{\rm col}$\tablenotemark{a} & Ab\tablenotemark{a,b}  &
$T_{\rm ex}$  & $N_{\rm col}$\tablenotemark{c} & Ab\tablenotemark{b,c}  &
$T_{\rm ex}$  & $N_{\rm col}$\tablenotemark{c} & Ab\tablenotemark{b,c}  &
                $N_{\rm col}$\tablenotemark{c} & Ab\tablenotemark{b,c}  \\
\hline
G10.34$-$0.14 &  21.9 &  49     &        6.8     &        3.8     &         &    $<$ 4.7     &    $<$ 2.6     &         &    $<$ 3.1     &    $<$ 1.7     &    $<$0.38     &    $<$0.21     \\
G11.92$-$0.61 &  54.5 &  75     &        4.0     &        1.1     &         &    $<$ 2.3     &    $<$ 0.6     &         &    $<$ 1.5     &    $<$ 0.4     &    $<$0.18     &    $<$0.05     \\
G12.20$-$0.03 &  31.3 &         & $\sim$ 3.6$^*$ & $\sim$ 2.0$^*$ &         &    $<$ 3.8     &    $<$ 2.1     &         &    $<$ 2.5     &    $<$ 1.4     &    $<$0.30     &    $<$0.17     \\
G12.42$+$0.50 &  94.9 &  29     &        2.1     &        1.9     &         &    $<$ 0.9     &    $<$ 0.8     &         &    $<$ 0.6     &    $<$ 0.5     &    $<$0.07     &    $<$0.06     \\
G12.68$-$0.18 &  39.1 & 102     &        7.4     &          -     &         & $\sim$ 8.0     &          -     &         & $\sim$ 1.4     &          -     & $\sim$0.79     &          -     \\
G12.91$-$0.03 &  19.5 &         & $\sim$ 4.4$^*$ & $\sim$ 1.6$^*$ &         &    $<$ 1.6     &    $<$ 0.6     &         &    $<$ 1.0     &    $<$ 0.4     &    $<$0.13     &    $<$0.05     \\
G12.91$-$0.26 &  70.1 &  76     &        9.6     &        1.0     & 109     &       15.9     &        1.7     & 100     &        3.1     &        0.3     & $\sim$0.51     & $\sim$0.05     \\
G14.33$-$0.64 &  28.8 &  53     &       12.9     &        4.8     &  70     &       14.1     &        5.2     &         &    $<$ 1.9     &    $<$ 0.7     &    $<$0.21     &    $<$0.08     \\
G14.63$-$0.58 &  20.1 &  38     &        3.9     &        4.8     &         &    $<$ 4.0     &    $<$ 5.0     &         &    $<$ 2.5     &    $<$ 3.1     &    $<$0.31     &    $<$0.39     \\
G16.59$-$0.05 &  25.5 &  82     &        9.5     &        4.3     &         & $\sim$11.2     & $\sim$ 5.1     &         &    $<$ 2.1     &    $<$ 1.0     &    $<$0.26     &    $<$0.12     \\
G18.89$-$0.47 &  20.8 &  46$^*$ &        2.9$^*$ &        1.7$^*$ &         &    $<$ 3.4     &    $<$ 2.0     &         &    $<$ 2.1     &    $<$ 1.2     &    $<$0.26     &    $<$0.15     \\
G19.01$-$0.03 &  60.6 & 111     &        1.6     &        0.6     &         &    $<$ 1.2     &    $<$ 0.5     &         &    $<$ 0.7     &    $<$ 0.3     &    $<$0.09     &    $<$0.03     \\
G19.36$-$0.03 &  27.9 &  34     &        3.6     &        0.5     &         &    $<$ 2.7     &    $<$ 0.4     &         &    $<$ 1.6     &    $<$ 0.2     &    $<$0.20     &    $<$0.03     \\
G19.88$-$0.53 &  46.4 &  55     &        5.4     &       10.8     &         &    $<$ 1.7     &    $<$ 3.4     &         &    $<$ 1.0     &    $<$ 2.0     &    $<$0.12     &    $<$0.24     \\
G22.04$+$0.22 &  19.5 &  81     &        5.9     &        1.9     &         &    $<$ 5.2     &    $<$ 1.7     &         &    $<$ 3.4     &    $<$ 1.1     &    $<$0.38     &    $<$0.12     \\
G23.01$-$0.41 &  37.2 & 101     &        9.1     &        1.7     &         & $\sim$ 7.2     & $\sim$ 1.3     &         &    $<$ 1.7     &    $<$ 0.3     & $\sim$0.73     & $\sim$0.13     \\
G23.96$-$0.11 &  30.6 &  27     &        2.7     &          -     &         &    $<$ 2.5     &          -     &         &    $<$ 1.4     &          -     &    $<$0.18     &          -     \\
G24.00$-$0.10 &  13.7 &  37     &        6.2     &        1.6     &         &    $<$ 7.1     &    $<$ 1.9     &         &    $<$ 4.2     &    $<$ 1.1     &    $<$0.52     &    $<$0.14     \\
G24.33$+$0.14 &  23.0 & 104     &        9.2     &          -     &  97     &       14.0     &          -     &         & $\sim$ 5.8     &          -     & $\sim$0.71     &          -     \\
G24.63$+$0.15 &  16.3 &         & $\sim$ 1.9     & $\sim$ 0.5     &         &    $<$ 3.5     &    $<$ 0.8     &         &    $<$ 2.2     &    $<$ 0.5     &    $<$0.28     &    $<$0.07     \\
G24.94$+$0.07 &  33.7 &         & $\sim$ 3.5$^*$ & $\sim$ 1.4$^*$ &         &    $<$ 1.8     &    $<$ 0.7     &         &    $<$ 1.1     &    $<$ 0.4     &    $<$0.14     &    $<$0.05     \\
G25.38$-$0.15 &  15.3 &  31     &        6.1     &        1.3     &         &    $<$ 4.3     &    $<$ 0.9     &         &    $<$ 2.8     &    $<$ 0.6     &    $<$0.35     &    $<$0.08     \\
G34.26$+$0.15 & 138.9 &  33     &        4.5     &        1.7     &         & $\sim$ 3.0     & $\sim$ 1.1     &         &    $<$ 0.9     &    $<$ 0.3     &    $<$0.10     &    $<$0.04     \\
G34.39$+$0.22 &  39.5 &         & $\sim$ 1.2     & $\sim$ 1.0     &         &    $<$ 1.7     &    $<$ 1.4     &         &    $<$ 1.1     &    $<$ 0.9     &    $<$0.13     &    $<$0.11     \\
G34.41$+$0.24 &  24.1 &  82     &       24.9     &       10.4     &  85     &       26.9     &       11.2     &  39     &       30.6     &       12.7     & $\sim$1.30     & $\sim$0.54     \\
G35.03$+$0.35 &  65.6 &  63     &        2.9     &        2.2     &         &    $<$ 2.5     &    $<$ 1.9     &         &    $<$ 1.5     &    $<$ 1.2     &    $<$0.18     &    $<$0.14     \\
G35.13$-$0.74 &  27.2 &  57     &        6.1     &        4.7     &         &    $<$ 4.2     &    $<$ 3.2     &         & $\sim$ 2.5     & $\sim$ 1.9     &    $<$0.30     &    $<$0.23     \\
G35.20$-$0.74 &  73.7 &  72     &        9.7     &        8.8     &         & $\sim$ 6.8     & $\sim$ 6.1     &         &    $<$ 1.8     &    $<$ 1.6     &    $<$0.18     &    $<$0.16     \\
G35.79$-$0.17 &  15.6 &  79     &       11.2     &          -     &         &    $<$ 9.0     &          -     &         &    $<$ 5.5     &          -     &    $<$0.69     &          -     \\
G39.10$+$0.49 &  24.7 &         & $\sim$ 1.6     & $\sim$ 2.3     &         &    $<$ 4.5     &    $<$ 6.5     &         &    $<$ 2.7     &    $<$ 3.9     &    $<$0.33     &    $<$0.47     \\
G39.39$-$0.14 &  25.1 & 105$^*$ &        3.9$^*$ &        2.4$^*$ &         &    $<$ 2.8     &    $<$ 1.7     &         &    $<$ 1.7     &    $<$ 1.0     &    $<$0.20     &    $<$0.13     \\
G40.28$-$0.22 &  33.9 &  58     &        7.4     &        4.9     &         &    $<$ 2.6     &    $<$ 1.7     &         &    $<$ 1.6     &    $<$ 1.1     &    $<$0.19     &    $<$0.13     \\
G45.47$+$0.05 &  35.5 &  37     &        2.0     &        1.8     &         &    $<$ 2.7     &    $<$ 2.5     &         &    $<$ 1.9     &    $<$ 1.7     &    $<$0.23     &    $<$0.20     \\
G45.80$-$0.36 &  18.2 &         & $\sim$ 2.7     &          -     &         &    $<$ 3.9     &          -     &         &    $<$ 2.3     &          -     &    $<$0.29     &          -     \\
G54.11$-$0.08 &  17.2 &         & $\sim$ 3.8     & $\sim$ 4.7     &         &    $<$ 4.8     &    $<$ 6.0     &         &    $<$ 2.9     &    $<$ 3.6     &    $<$0.36     &    $<$0.45     \\
G58.78$+$0.64 &  15.6 &         & $\sim$ 4.6     & $\sim$ 4.6     &         &    $<$ 7.6     &    $<$ 7.6     &         &    $<$ 4.5     &    $<$ 4.5     &    $<$0.56     &    $<$0.56     \\
G59.79$+$0.63 &  24.8 &  32     &        2.7     &        2.1     &         &    $<$ 4.6     &    $<$ 3.5     &         &    $<$ 2.7     &    $<$ 2.1     &    $<$0.34     &    $<$0.26     \\
\hline
\end{tabular*}
\tablenotetext{a}{Values preceded with `$\sim$' are estimated by assuming a median rotational temperature of 58\,K, as obtaind from  the other 28 stronger methanol emitters.}
\tablenotetext{b}{The abundance `Ab' is estimated with the H$_2$ column density estimated from C$^{18}$O by \citet{chen10}, while `-' means the lack of C$^{18}$O observation in that paper.}
\tablenotetext{c}{Values preceded with `$\sim$' and upper limits are estimated by adopting the mean rotation temperature of 90\,K of CH$_3$OCH$_3$.}
$^*$ These values of methanol are less reliable because several methanol lines are unexpecedly undetected on the rotation diagram.
\end{minipage}
\end{table*}

